Structured AI ideation yields physical strategies for epithelial barrier repair

AI systems increasingly support literature analysis, candidate evaluation and hypothesis refinement, but enabling researchers to explore research directions beyond established disciplinary approaches remains challenging. We developed Abelio, an AI system designed to generate novel research directions by expanding investigators' avenues of inquiry. Abelio reformulates research objectives, uses these alternative formulations to identify relevant elements outside conventional disciplinary boundaries, and refines the resulting hypotheses. Each stage integrates divergent exploration with convergent selection through a dedicated subsystem. In quantitative evaluations, proposals generated by the Ideation Core (Abelio's hypothesis-generation core) outperformed those of four frontier large language models in scientific soundness and hypothesis diversity, and three of four in distance from existing literature. Subsystem ablation showed that each subsystem contributes to the property it targets, with the contribution of Element Selection measurable before Refinement. To investigate intestinal epithelial barrier restoration, Abelio proposed physical interventions involving membrane-tethered poly(ethylene glycol) (PEG) and cholesterol-anchored complementary DNA. Both proposals were archived before experimentation and subsequently tested independently in damaged Caco-2 monolayers. PEG preserved barrier function in a membrane-surface-dependent manner, whereas complementary DNA enabled sequence-specific restoration that was reversible on demand. These findings demonstrate how structured research ideation can identify experimentally testable approaches beyond established disciplinary conventions.

==> justfile <==
set shell := ["fish", "-c"]

default:
	@just --list

format-bib:
	bibtool -r .bibtoolrsc -s -i references.bib -o references.bib.tmp
	mv references.bib.tmp references.bib

format-tex:
    for file in **/*.tex; latexindent --s -w -m -l indentconfig.yaml -g=/dev/null $file; perl -0777 -pe 's/\n+$/\n/' $file > $file.tmp && mv $file.tmp $file; end;
    rm **/*.bak*

format:
	@just format-bib
	@just format-tex

